SeaPearl: A Constraint Programming Solver guided by Reinforcement Learning

The design of efficient and generic algorithms for solving combinatorial optimization problems has been an active field of research for many years. Standard exact solving approaches are based on a clever and complete enumeration of the solution set. A critical and non-trivial design choice with such methods is the branching strategy, directing how the search is performed. The last decade has shown an increasing interest in the design of machine learning-based heuristics to solve combinatorial optimization problems. The goal is to leverage knowledge from historical data to solve similar new instances of a problem. Used alone, such heuristics are only able to provide approximate solutions efficiently, but cannot prove optimality nor bounds on their solution. Recent works have shown that reinforcement learning can be successfully used for driving the search phase of constraint programming (CP) solvers. However, it has also been shown that this hybridization is challenging to build, as standard CP frameworks do not natively include machine learning mechanisms, leading to some sources of inefficiencies. This paper presents the proof of concept for SeaPearl, a new CP solver implemented in Julia, that supports machine learning routines in order to learn branching decisions using reinforcement learning. Support for modeling the learning component is also provided. We illustrate the modeling and solution performance of this new solver on two problems. Although not yet competitive with industrial solvers, SeaPearl aims to provide a flexible and open-source framework in order to facilitate future research in the hybridization of constraint programming and machine learning.

==> content/Stateofart.tex <==
\section{Related work}
\qcap{Can be moved in the introduction or before the related work}
Before heading to our main contribution and to understand the scientific contest and the interest of this work, let's look at three previous successful attempts to learn how to solve COP problems, which inspired and motivated this project.  

\subsection{Learning solutions heuristics}

A first approach to learn how to solve has been to learn a solution heuristic directly. This means creating a solver in itself, in the form of a reinforcement learning agent taking a problem as input and retrieving a possible solution. This has been done by \cite{bello2017neural}, \cite{dai2018learning} or by \cite{deudoncournut2018}. In this case, Reinforcement Learning is not enhancing another solving method but is learning to solve directly. A great interest of this is that, once trained, it's very fast to find good approximations to new problems. But this approach has three drawbacks: first, it is very problem-specific. Then, there is no generic way to improve the result and to prove optimality. Finally, it's quite limited to simple problems and cannot handle properly constraints like Mixed Integer Programming and Constraint Programming do. 

Nevertheless, this has proved that Deep Reinforcement Learning can really bring improvement to COP solving and has motivated a lot of work in this new field.

\subsection{Learning value selection heuristics outside a solver}

In order to exploit the potential of reinforcement learning to find solutions, Q. Cappart \cite{cappart2020combining} chose to use one as a value selection heuristic inside a constraint programming solver. 

This new approach solves the shortcomings of previous approaches: the solver is much more general and robust, it can handle more complicated COPs and it can improve its solutions while increasing execution time and get the possibility to prove optimality. On the contrary, it keeps the power of Deep Reinforcement Learning for proposing interesting solutions soon in the solving and this way being able to prune the search space quite efficiently. It has proved its efficiency on the Travelling Salesman Problem with Time Windows (TSPTW - a constrained variant of the TSP) and the 4-moments portfolio optimization problem. It has been able to reduce the number of nodes visited compared to classic CP approach and previous DRL approaches and it has been able to find best solutions with the same execution time.

Even if also proven effective, the value selection heuristic learned might not be the best as it has been trained as a solution heuristic not a value selection heuristic. It has not been trained during a CP solving procedure, which means it has not had all the CP specific information available while training. It has only been trained to find a good solution and is not aware of CP problematics like proving optimality. Thus, we think that we could go even further and have heuristics learning more specifically to choose efficiently value during a CP procedure. This work has motivated our project to create a completely unified solver where the training could be entirely done inside the solver. 

\subsection{Learning heuristics inside the solver}

Finally, it's interesting to mention that learning inside a solver has already proven effective but without using deep reinforcement learning. This approach, presented in Impact-Based Search Strategies for Constraint Programming \cite{refalo2004impact} define a metric called Impact inspired by two principles used in handcrafted value and variable selection heuristics. The first principle is that the variable which assignment reduce the search space will reduce the search effort. The second principle is that a value that maximizes the number of possibilities for future assignment will help find solutions. 

Hence, a few assignments are used to estimate the impact of a variable and the impact of values and the search is oriented with this simple rule: we first choose variable with big impacts and we first branch on values with low impacts. This strategy has also been proven effective and is implemented in most of the recent solvers. If we look at this strategy, it is learned with "restricted rules" but it could well be learned by an agent in the reinforcement learning framework. The strategy learned could even be more efficient. The limitation could be the time needed to learn as this strategy is learned during a solving procedure and not in a previous training phase. 

In any case, this strategy shows that learning inside the solver gives access to very expressive metrics which can help building highly efficient variable and value selection heuristics.



==> content/StyleExample.tex <==
\section{First Section}
\subsection{A Subsection Sample}
Please note that the first paragraph of a section or subsection is
not indented. The first paragraph that follows a table, figure,
equation etc. does not need an indent, either.

Subsequent paragraphs, however, are indented.

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
\includegraphics[width=\textwidth]{fig1.eps}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}
